EmoTrack: An application to Facilitate User Reflection on Their Online Behaviours

With the rapid growth of the internet, all online activities can have both positive and negative effects on human mental health. Online engagement is complex and efforts to regulate online use face challenges in distinguishing between beneficial and harmful content and behaviours. An alternative approach is to help young people develop the skills they need to manage online safety while preserving the benefits of online interactions. This dissertation presents the entire development process and evaluation of an multi-platform application, called EmoTrack that aims to help young people reflect on their online behaviour. It was developed to record their online activities and cultivate strategies for more positive and mindful engagement online. EmoTrack is a personal informatics system, and it is designed to help people track and reflect on their engagement with YouTube videos. The system was evaluated with thirteen participants and it was found that EmoTrack can facilitate them to reflect on their video watching behaviour and the impact on their mood, with reports of different levels of reflections from R0 to R3.

==> Makefile <==
SHELL := /bin/bash

SOURCES = $(wildcard *.tex)
TARGETS = $(patsubst %.tex, %.pdf, ${SOURCES})

TEXMFLOCAL = "/home/crypto/texmf"

${TARGETS} : %.pdf : %.tex $(wildcard %.bib)
	@for i in `seq 3`                           ; do   \
           TEXMFLOCAL="${TEXMFLOCAL}" pdflatex ${*} ;      \
           if grep -q "bibliography" ${*}.tex       ; then \
             TEXMFLOCAL="${TEXMFLOCAL}" bibtex ${*} ;      \
           fi                                       ;      \
         done

all      : ${TARGETS}

clean    :
	@rm -f *.{aux,bbl,blg,loa,lof,log,lol,lot,nav,out,snm,toc}

spotless : clean
	@rm -f ${TARGETS}

.DEFAULT_GOAL := all

